Macro2Micro: A Rapid and Precise Cross-modal Magnetic Resonance Imaging Synthesis using Multi-scale Structural Brain Similarity

The human brain is a complex system requiring both macroscopic and microscopic components for comprehensive understanding. However, mapping nonlinear relationships between these scales remains challenging due to technical limitations and the high cost of multimodal Magnetic Resonance Imaging (MRI) acquisition. To address this, we introduce Macro2Micro, a deep learning framework that predicts brain microstructure from macrostructure using a Generative Adversarial Network (GAN). Based on the hypothesis that microscale structural information can be inferred from macroscale structures, Macro2Micro explicitly encodes multiscale brain information into distinct processing branches. To enhance artifact elimination and output quality, we propose a simple yet effective auxiliary discriminator and learning objective. Extensive experiments demonstrated that Macro2Micro faithfully translates T1-weighted MRIs into corresponding Fractional Anisotropy (FA) images, achieving a 6.8\% improvement in the Structural Similarity Index Measure (SSIM) compared to previous methods, while retaining the individual biological characteristics of the brain. With an inference time of less than 0.01 seconds per MR modality translation, Macro2Micro introduces the potential for real-time multimodal rendering in medical and research applications. The code will be made available upon acceptance.

==> Table/ADHD_classification.tex <==
\begin{table}[t!]
  \small \centering
  \caption{ADHD classification performance of real T1, real FA, and generated FA images.}
  \label{tab:ADHD classification}
  \renewcommand{\arraystretch}{1.1}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{ccccc}
    \toprule
    \hline
    Input & AUROC ($\uparrow$) & ACC ($\uparrow$) \\ \hline
    \midrule 
    T1 &  0.5034          & 0.5479 \\
    FA (GT) &  0.4812          & 0.5342   \\ \hdashline
    Pix2Pix FA &  \textbf{0.5532}          & \textbf{0.5821}   \\
    Cycle GAN FA &  0.4445          & 0.4794  \\ \hline
    Ours (Macro2Micro FA)  &  \textbf{0.4926}           & \textbf{0.5136}    \\
    \hline
    \toprule 
    \end{tabular}}
\end{table} 

==> Table/baseline_onlyWM.tex <==
\begin{table}[t!]
  \small \centering
  \caption{Quantitative comparison with baseline models using only white matter whose FA value is bigger than 0.2 from the generated FA images.}
  \label{tab:baseline_onlyWM}
  \renewcommand{\arraystretch}{1.1}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{ccccc}
    \toprule
    \hline
    Methods & SSIM ($\uparrow$) & PSNR ($\uparrow$) & MAE ($\downarrow$)& MSE($\downarrow$) \\ \hline
    \midrule 
    Pix2Pix & 0.8354 & 24.8992 & 0.1374 & 0.1200 \\
    Cycle GAN & 0.8369 & 24.7585 & 0.1383 & 0.1208 \\ \hline
    Ours (Macro2Micro) & \textbf{0.8627} & \textbf{25.8493} & \textbf{0.1300}& \textbf{0.1146} \\
    \hline
    \toprule 
    \end{tabular}}
\end{table} 

==> Table/baseline_wholebrain.tex <==
\begin{table}[t!]
  \small \centering
  \caption{Quantitative comparison with generated whole brain FA images. The best outcomes are shown in \textbf{bold}. ↑: Higher is better. ↓: Lower is better.}
  \label{tab:baseline_wholebrain}
  \renewcommand{\arraystretch}{1.1}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{ccccc}
    \toprule
    \hline
    Methods & SSIM ($\uparrow$) & PSNR ($\uparrow$) & MAE ($\downarrow$)& MSE($\downarrow$) \\ \hline
    \midrule 
    Pix2Pix & 0.8310 & 24.7738 & 0.1469 & 0.1292 \\
    Cycle GAN & 0.8332 & 24.6660 & 0.1477 & 0.1299 \\ \hline
    Ours (Macro2Micro) & \textbf{0.8600} & \textbf{25.7560} & \textbf{0.1383}& \textbf{0.1226} \\
    \hline
    \toprule 
    \end{tabular}}
\end{table} 


==> Table/brain_PD.tex <==
\begin{table}[t!]
  \small \centering
  \caption{\textbf{Ablation study} for brain-focused patch discriminator.}
  \label{tab:brain_PD}
  \renewcommand{\arraystretch}{1.1}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{ccccc}
    \toprule
    \hline
    Methods & SSIM ($\uparrow$) & PSNR ($\uparrow$) & MAE ($\downarrow$)& MSE($\downarrow$) \\ \hline
    \midrule 
    No brain PD & \textbf{0.8663} & \textbf{26.2560} & 0.1440 & 0.1288 \\
    Macro2Micro & \textbf{0.8631} & \textbf{26.0478} & \textbf{0.1374}& \textbf{0.1221} \\
    \hline
    \toprule 
    \end{tabular}}
\end{table} 

==> Table/intelligence_regression.tex <==
\begin{table}[t!]
  \small \centering
  \caption{Intelligence regression performance of real T1, real FA, and generated FA images.}
  \label{tab:intelligence classification}
  \renewcommand{\arraystretch}{1.1}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{ccccc}
    \toprule
    \hline
    Input & Corr. Coef. ($\uparrow$) & MSE ($\downarrow$) \\ \hline
    \midrule 
    T1 &  0.159          & 0.777 \\
    FA (GT) &  0.124          & 0.832   \\ \hdashline
    Pix2Pix FA &   \textbf{0.187}         & \textbf{0.784}   \\
    Cycle GAN FA &  0.066         &     0.836  \\ \hline
    Ours (Macro2Micro FA)  &  \textbf{0.166}           & \textbf{0.797}    \\
    \hline
    \toprule 
    \end{tabular}}
\end{table} 

==> Table/norm_relu.tex <==
\begin{table}[t!]
  \small \centering
  \caption{\textbf{Ablation study} for different normalization and activation functions.}
  \label{tab:norm_relu}
  \renewcommand{\arraystretch}{1.1}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{ccccc}
    \toprule
    \hline
    Methods & SSIM ($\uparrow$) & PSNR ($\uparrow$) & MAE ($\downarrow$)& MSE($\downarrow$) \\ \hline
    \midrule 
    Batch Norm & 0.8521 & 25.4675 & 0.1425 & 0.1258 \\
    Instance Norm & 0.8605 & 25.8663 & 0.1419 & 0.1260 \\
    ReLU & 0.8575 & 25.8609 & 0.1399 & 0.1242 \\ \hline
    Macro2Micro & \textbf{0.8631} & \textbf{26.0478} & \textbf{0.1374}& \textbf{0.1221} \\
    \hline
    \toprule 
    \end{tabular}}
\end{table} 

==> Table/octave.tex <==
\begin{table}[t!]
  \small \centering
  \caption{\textbf{Ablation study} Depending on whether Octave Convolution is applied and the difference in $\alpha$ value.}
  \label{tab:Octave}
  \renewcommand{\arraystretch}{1.1}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{cccccc}
    \toprule
    \hline
    Methods & SSIM ($\uparrow$) & PSNR ($\uparrow$) & MAE ($\downarrow$)& MSE($\downarrow$) & Time($\downarrow$) \\ \hline
    \midrule 
    No Octave & 0.8598 & 25.8797 & \textbf{0.1280} & \textbf{0.1122} & \textbf{0.0056} \\
    Oct \alpha=0.25 & \textbf{0.8640} & \textbf{26.1565} & 0.1417 & 0.1264 & 0.0126 \\
    Oct \alpha=0.75 & 0.8597 & 25.9887 & 0.1414 & 0.1258 & 0.0129 \\ \hline
    Macro2Micro (\alpha=0.50) & \textbf{0.8631} & \textbf{26.0478} & \textbf{0.1374}& \textbf{0.1221} & \textbf{0.0110}\\
    \hline
    \toprule 
    \end{tabular}}
\end{table} 

==> Table/sex_classification.tex <==
% \begin{table}
% \begin{tabular}{lll}
% sex                & AUROC           & Accuracy \\
% T1                 & 0.7820          & 0.7133   \\
% FA (GT)           & 0.7641          & 0.7066   \\
% CycleGAN FA           & 0.7534          & 0.6766   \\
% Pix2Pix FA            & 0.7565          & 0.68     \\ \hline
% Ours (Macro2micro FA) & \textbf{0.7726} & 0.6866  
% \end{tabular}
% \label{tab:sex classification}
% \end{table}'


\begin{table}[t!]
  \small \centering
  \caption{Sex classification performance of real T1, real FA, and generated FA images. GT: Ground Truth.}
  \label{tab:sex classification}
  \renewcommand{\arraystretch}{1.1}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{ccccc}
    \toprule
    \hline
    Input & AUROC ($\uparrow$) & ACC ($\uparrow$) \\ \hline
    \midrule 
    T1 &  0.7820          & 0.7133 \\
    FA (GT) &  0.7641          & 0.7066   \\ \hdashline
    Pix2Pix FA &  0.7565          & 0.68   \\
    Cycle GAN FA &  0.7534          & 0.6766  \\ \hline
    Ours (Macro2Micro FA)  &  \textbf{0.7726}           & \textbf{0.6866}    \\
    \hline
    \toprule 
    \end{tabular}}
\end{table} 




==> Table/vgg_loss.tex <==
\begin{table}[t!]
  \small \centering
  \caption{\textbf{Ablation study} of perceptual loss using pre-trained VGG network.}
  \label{tab:vgg}
  \renewcommand{\arraystretch}{1.1}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{ccccc}
    \toprule
    \hline
    Methods & SSIM ($\uparrow$) & PSNR ($\uparrow$) & MAE ($\downarrow$)& MSE($\downarrow$) \\ \hline
    \midrule 
    No VGG loss & 0.8565 & 25.7207 & 0.1407 & 0.1251 \\
    Macro2Micro & \textbf{0.8631} & \textbf{26.0478} & \textbf{0.1374}& \textbf{0.1221} \\
    \hline
    \toprule 
    \end{tabular}}
\end{table} 

==> redun./INTRO______.tex <==
% Introduction 문단 구조
1. 인간 뇌의 구조적 가소성
2. 연구 문제
3. Modality, Frequency 설명 및 연관성
    - Macro, Micro에 해당하는 MRI modality 설명 및 사용 예시
    - Frequency & brain의 Macro, Micro의 연관성
4. clinical 효과
    - 시간, 비용 단축
    - B-value가 커지면 noise가 심해지기 때문에 denoising
    - diffusion tensor imaging and tractography
also suffer from well described methodological and technical limitations that often lead to artifacts and potential errors in the assessment [The CONNECT project: Combining macro- and micro-structure]
5. 딥러닝
-----
1. 사람의 뇌는 바뀐다. 우리 뇌의 구조적 변경성

2.  과연 이런 구조적 변화의 원인은 어디서 비롯? 결국 macro. macro는 static, micro는 dynamic// 결국 micro 변화는 macro에서부터 비롯된다. (rationale? 근거가 없어도 우리가 그런 방향을 찾는다) // macro에서 마이크로 가는건 되게 중요한데 아직 그런 연구가 잘 없었다.  구조로부터 기능을 엮을 수 있다는 것. 이것이 풀고 싶은 숙제다. 이걸 알기 위해 매크로한 구조에서 마이크로한 구조를 예측해보는 것에서 이를 검증해보고자 한다.

3. 모달리티 설명 등 // 매크로 마이크로 구조 설명
3. (실용성) 디퓨전 때문에 마이크로 구조기 때문에 노이즈도 많고 찍기도 어렵다. —> 노이즈로부터 조금 더 robust

4. 이런 시도가 있었다.
5. 그래서 이걸 딥러닝 써서 해보려고한다. (이유) 그리고 뭘 이루어냈다 (간단하게) frequency 정보 나눠서 한다

3번에서 두개의 모달리티가 다르다.
------

The brain consists of multiple brain regions that carry out distinct functions and are interconnected by neural pathways~\cite{friston2004functional}. Specifically, the functioning of the human brain is predominantly influenced by its neural connections. Nevertheless, these neuronal connections are not fixed but continuously modified at both systemic and synaptic levels throughout one's lifetime to efficiently accommodate the dynamic environment. This dynamic modification of its structure at the macro- and micro-scale of the human brain is called \textit{structural plasticity}.

The macro-structure of the human brain refers to the architecture of cell bodies and neurite arrangement within the gray matter or axonal properties (e.g., tissue organization, size distribution, density, and myelin content) in the white matter. The macro-structure of the human brain has enormous potential in understanding the structure and organization of the brain, providing unique insights for abnormalities that underpin disease states. With the advent of Magnetic Resonance Imaging (MRI), the macro-structure of the human brain could be captured by structural MRIs (sMRI), especially with T1-weighted MRI. This is because T1-weighted images mainly depict the overall shape or size of the brain tissues.

The micro-structure, on the other hand, refers to the microscopic structure of brain tissue components such as myelin, axons, and dendrites or the quantification of their properties. This microscopic architecture includes multiple properties such as cell size, the orientation of axonal fiber bundles, or packing density. Recently, diffusion MRI (dMRI) models such as Diffusion-Weighted Image (DWI) have primarily been used for studying brain tissue micro-structures\cite{gu2019generating} and helping recognize tissue damage or abnormalities that depend on the cell density of the tissue. Providing rich information about micro-structural characterization, DWI is also used in many advanced dMRI models such as neurite orientation dispersion and density imaging (NODDI) or diffusion tensor imaging (DTI).

As both macro- and micro-structure of the brain convey different yet complementary information about the human brain, considering both structures simultaneously is extremely important for understanding the \texdit{structural plasticity} of the human brain and neuronal connectivity during cognitive tasks and allows for a more comprehensive understanding of brain information. For instance, DTI is particularly sensitive in reflecting the structural state of white matter, which has led to active research in white matter diseases such as multiple sclerosis \cite{horsfield1996apparent, roosendaal2009regional}, CADASIL\cite{chabriat1999clinical, o2005damage}, and Alzheimer's disease\cite{mayo2019relationship, chen2023abnormal}. These studies have demonstrated that DTI can faithfully detect pathological alterations in white matter regions that appear normal in T1-weighted MRI and show that changes in DTI measures correlate with pathological changes and clinical findings.

There have been numerous attempts to integrate these modalities that encode different structural scales of human brain information in a multimodal fashion in neuroimaging studies. However, multimodal deep learning poses several crucial challenges. First, obtaining such modalities is \textit{extremely} costly and time-consuming.





Moreover, research to use tractography, which can faithfully provide brain connection information on the finest scale, is also in the spotlight. The diffusion-derived scalar maps like Fractional Anisotropy (FA) 











The macro-structure of the human brain refers to the architecture of cell bodies and neurite arrangement within the gray matter or axonal properties (e.g., tissue organization, size distribution, density, and myelin content) in the white matter. The macro-structure of the human brain has enormous potential in understanding the structure and organization of the brain, providing unique insights for abnormalities that underpin disease states. The micro-structure, on the other hand, refers to the microscopic structure of brain tissue components such as myelin, axons, and dendrites or the quantification of their properties. This microscopic structural architecture includes multiple properties such as cell size, the orientation of axonal fiber bundles, or packing density. %Several dysfunctions of the human brain result from pathological features such as demyelination, inflammation, and axonal loss~\cite{cercignani2018brain}. 
As both macro- and micro-structure of the brain convey different yet complementary information of the human brain, considering both structures is extremely important for understanding the \textit{structural plasticity} of the human brain and neuronal connectivity during cognitive tasks.

With an advent of Magnetic Resonance Imaging (MRI), 




%%%%%%%%%%%%%%%%%%%%%%%%%% 1. 인간 뇌의 구조적 가소성 %%%%%%%%%%%%%%%%%%%%%%%%%%
인간의 뇌는 connectivity로 정의, 연결된다.
-> 이건 '주어진 환경에 맞게' '적응'하는 과정에서 끊임없이 변경 


사람 뇌는 다양한 기능을 하는 영역들과 연결성으로 이루어져있다. 뇌의 영역들은 local한 기능을 하기도 하며 다른 영역들과의 neural connection을 가지고 상호작용 하고 있다. 뇌의 구조와 그 구조들 간의 connectivity는 

The human brain is primarily defined by segregated brain regions and their connections. The brain regions have highly localized functions that reflect neural characteristics and interact with other regions through neural connections. 



%%%%%%%%%%%%%%%%%%%%%%%%%% 2. 뇌의 Macro, Micro %%%%%%%%%%%%%%%%%%%%%%%%%%
<기존>
-> 이를 가능하게 하는 것은  macro/micro level의 '구조적' 가소성 (기능적 가소성을 굳이 언급 안하는게 명확할듯) 
-> macro/micro 설명 + 각각을 측정하는 modalitity 소개
-> 각각이 뇌에서 갖는 의미와 표상하는 정보가 다르다는 것을 주장. 
-> 그래서 이를 통합하기 위한 multimodal 연구들이 많이 이루어졌다

구조적인 변화의 방향이 macro로부터 나올 수 있다 -> 확인 필요
그래서 macro로부터 micro를 만들어낼 수 있다는 것을 입증할 수 있다
Macro는 잘 안바뀌고 오래 걸리는데(static) dynamic한 micro한 정보는 Macro한 정보를 바탕으로 변화할 수밖에 없다.
macro에서 마이크로 가는건 되게 중요한데 아직 그런 연구가 잘 없었다. 구조로부터 기능을 엮을 수 있다는 것. 이것이 풀고 싶은 숙제다. 
이걸 알기 위해 매크로한 구조에서 마이크로한 구조를 예측해보는 것에서 이를 검증해보고자 한다.

    1) Macro structure는 잘 바뀌지 않는다.
    2) Micro structure or connectivity는 보다 쉽게 바뀐다.
    3) 

microstructure is important for understanding cognition and disease




%%%%%%%%%%%%%%%%%%%%%%%%%% 3. Modality & Frequency %%%%%%%%%%%%%%%%%%%%%%%%%%

For structural connectivity analysis, in particular, diffusion MRI (dMRI) and tractography algorithms (see (Behrens and Jbabdi, 2009) for a review) have allowed novel explorations of inter-regional pathways in the living brain.

==> redun./Redundant.tex <==
To further test the robustness and effectiveness of the proposed model, we conducted principal component analysis (PCA) and T-SNE on three types of images: T1-weighted images, ground truth FA images, and synthesized FA images. We analyzed and visualized 1,499 subjects in the test dataset. After flattening $256^2$ voxels from MRI slices, we removed the non-brain background, leaving 26,891 voxels for each brain modality, PCA and T-SNE were then applied to the entire features. A batch size of 200 was utilized for the incremental PCA, a learning rate of 100 and perplexity of 30 were applied in the T-SNE algorithm, and the visualization was performed using two principal components. In the case of PCA, the two principal components individually accounted for 13.7 \% and 2.7 \% of the variances. Notably, both PCA and T-SNE demonstrated that the generated FA images exhibited significant dissimilarity compared to the original T1 images while displaying an overlap with the ground truth FA images in the low-dimensional representation (Fig.~\ref{fig:PCA TSNE macro2micro}).



%우리 모델의 결과가 실제 tractography image와 비교했을 때 가장 유사했다. In Figure~\ref{fig:phase2}, vmPFC 영역을 지나는 fiber가 지나가는 전체적인 위치와 streamline이 많이 지나다니는, 밀집되어 있는 region은 잘 예측하였다. target tractography 주위에 원본에는 없는 noise를 더 많이 만들어내는 Pix2Pix와 CycleGAN과 비교했을 때, noise가 거의 없으며 region 예측이 훨씬 정확하다. SSIM, PSNR, MAE and MSE에서도 훨씬 높은 performance score를 보였다 (Table~\ref{tab:phase2}).


% 결과 해석
% 원본) 우리 이미지는 T1에서부터 구조적인 정보를 보존하며 FA를 만들기 때문에 다른 모델들을 통해 만든 이미지뿐만 아니라 심지어 종종 GT보다 구조적인 정보를 high-resolution으로 만들어낸다. 다른 모델들처럼 input과 output 사이의 mapping만 학습 하는것이 아니라 input의 macro-scturture 구조를 유지한채로, 인지한채로 micro-structure를 학습한다고 추론할 수 있다. GT FA에도 없는, 끊겨있는, 뭉개져있는 위치의 white matter 구조를 보다 정확하게 high-resolution으로 만들어내는데 이는 우리 모델이 macro-scale과 micro-scale 구조간의 연관성을 학습하여 GT FA에서 부족한 정보를 T1으로부터 얻어와 더욱 microscophic white matter를 생성한다는 것을 알 수 있다. 또한, micro structure를 생성할 때 microscophic 정보만 필요한 것이 아니라 macro-scale의 정보가 도움이 된다는 것을 입증했다.
% 상윰버전) 우리 모델은 T1의 구조적인 정보를 보존해서 FA를 만들기 때문에 generated FA가 ground truth FA와 높은 수준으로 일치함은 물론이고, 종종 ground truth FA image가 가지고 있는 구조적인 정보보다 더 높은 resolution으로 정보를 생성하기도 한다. ground truth FA에서 발견되지 못하는 끊겨져있거나 뭉개져있는 위치의 white matter 구조를 보다 정확하게 high-resolution으로 만들어내는데 이는 우리 모델이 macro-scale과 micro-scale 구조간의 연관성을 학습할 뿐만 아니라 Ground truth FA에서 부족한 정보를 T1으로부터 얻어와 더욱 정확한 microscophic white matter를 생성한다는 것을 알 수 있다.
Our model preserves the structural information from T1 to generate FA, resulting in generated FA images that not only exhibit a high level of agreement with the ground truth FA but often surpass it in terms of structural information at a high resolution. It accurately generates high-resolution white matter structures in locations where the ground truth FA exhibits disconnected or distorted regions. This indicates that our model learns the association between macro-scale and micro-scale structures, allowing it to extract additional information from T1 that is missing in the ground truth FA, resulting in a more accurate generation of microscopic white matter structures. It demonstrates that macro-scale knowledge is useful for designing micro-structures, in addition to micro-scale information.
\\
% 일상생활 데이터와 다르게 brain image는 gray scale로 색깔에 대한 정보보다 structure, contrast와 edge와 같은 정보에 집중되어 있다. Image를 high frequency와 low frequency로 나눠서 인지하는 Octave Convolution을 이용했을 때, brain image의 퀄리티를 결정하는 contrast와 structure 같은 특성들을 frequency 영역으로 나눠서 더 효율적으로 잘 encoding하고 generating 할 수 있다.
% 상윰버전) computer vision 분야에서 일반적으로 접할 수 있는 RGB 값을 가지는 이미지 데이터와 다르게 brain image는 gray scale로 이루어져있고, 색깔에 대한 정보보다 structure, contrast와 edge와 같은 형태 정보에 집중되어 있다. 따라서 Image를 high frequency와 low frequency로 나눠서 encoding하는 Octave Convolution을 이용했을 때, brain image의 퀄리티를 결정하는 contrast와 structure 같은 특성들을 효율적으로 잘 encoding하고 generating 할 수 있다.

Unlike natural images that can be easily encountered in the computer vision domain, brain images focus more on structural information, contrast, and edges rather than color information. Octave Convolution, which divides images into high-frequency and low-frequency components, can be used to efficiently encode and generate brain images, effectively maintaining high image qualities such as contrast or structure.

% brain image가 가지는 특성이 일반적으로 computer vision에서 사용하는 데이터와 많이 달라서 pre-trained를 쓰지 않고 학습을 새로 시키는 경우가 많다. 그러나, 일반 데이터로 pretrained된 VGG를 사용해 perceptual loss를 구한 결과, 이미지에서 나타나던 skull 형태의 artifact를 없앨 수 있었다. 이를 통해 일반 데이터와 brain image가 어느 정도의 level에서는 유사한 특징을 공유한다고 추론해 볼 수 있다. 이를 통해 일반 데이터로 pretrained된 모델의 brain domain으로 확장 가능성을 확인한다.
% 상윰버전) 앞서 서술한 대로 brain image가 가지는 특성이 일반적으로 computer vision에서 사용하는 데이터와 많이 다르기 때문에 pre-trained model을 사용하지 않고 학습을 새로 시키는 경우가 많다. 그러나, 일반적인 이미지 데이터로 pretrained된 VGG를 사용해 perceptual loss를 구한 결과, 이미지에서 나타나던 skull 형태의 artifact를 없앨 수 있었다. 이를 통해 일반 데이터와 brain image가 어느 정도의 level에서는 유사한 특징을 공유한다고 추론해 볼 수 있다. 이를 통해 일반 데이터로 pretrained된 모델의 brain domain으로 확장 가능성을 확인할 수 있었다.
When dealing with brain images, it is common to train models from scratch rather than relying on pre-trained models. However, the pre-trained VGG model with computer vision data used for perceptual loss of images removes skull-shaped artifacts in the FA images. This suggests that, on some level, generic image data and brain images may share image features. This finding indicates the potential for extending pre-trained models from general data to the brain domain, opening up possibilities for further exploration.
\\

% brain image는 배경이 많은 부분을 차지하기 때문에 배경의 loss값이 작더라도 차지하는 pixel의 비율이 커 학습의 target이 되어야하는 뇌 안의 영역이 잘 학습되지 않는 경우가 있다. 이를 해결하기 위해 brain을 더 확대해 실제인지 아닌지 판단하는 patch discriminator를 적용하여 brain 영역의 loss에 focus하였다. 생성된 이미지의 detail한 부분의 resolution이 높아졌으며 brain의 boundary에 발생하던 checkerboard나 dotted line과 같은 artifact가 발생하지 않았고 brain boundary가 실제와 더 유사해졌다. 배경과 전반적인 image quality는 pixel loss나 vgg perceptual loss로 충분히 학습할 수 있으며 뇌 이미지의 artifact와 microscophic quality는 brain-focus Patch Discriminator를 통해 개선했다고 볼 수 있다.
% 상윰버전) brain image는 배경이 많은 부분을 차지하기 때문에 배경의 loss값이 작더라도 차지하는 pixel의 비율이 커 학습의 target이 되어야하는 뇌 안의 영역이 잘 학습되지 않는 경우가 있다. 이를 해결하기 위해 brain을 확대하고 patch로 쪼개서 해당 patch가 실제 데이터인지 아닌지 판단하는 patch discriminator를 적용하여 brain 영역의 loss에 focus하였다. 결과적으로 생성된 이미지의 detail한 부분의 resolution이 높아졌으며 brain의 boundary에 발생하던 checkerboard나 dotted line과 같은 artifact가 발생하지 않았고, brain boundary가 실제와 더 유사해졌다. 배경과 전반적인 image quality는 pixel loss나 vgg perceptual loss로 충분히 학습할 수 있으며 뇌 이미지의 artifact와 microscophic quality는 brain-focus Patch Discriminator를 통해 개선했다고 볼 수 있다.
In most cases, the brain images include a significant portion of the redundant background. Even if the loss values of background are small, the background potentially impedes the learning of the brain region. A patch discriminator is employed to address this problem by cropping the image around the brain. The patch discriminator extracts patches from images and determines whether each patch belongs to the actual brain data or not. This approach focused on the loss of only brain regions during training. As a result, the quality of generated images gets higher in the detailed region, and artifacts such as checkerboard patterns or dotted lines at the brain boundary could be effectively solved. The brain boundary becomes more similar to the actual boundaries. Background and overall image quality can be adequately learned using pixel loss and VGG perceptual loss. 

Microscopic quality and artifacts specific to brain images are improved by the brain-focused Patch Discriminator. This approach helps to alleviate the challenges posed by the background dominance and allows the model to better capture and generate high-quality brain images with improved details, accuracy in brain region representation, and reduced artifacts.
 
% Macro2Micro에서 생성된 FA 이미지의 Sex classification 예측 성능이 실제 FA 이미지보다 예측된 것은 여러 측면에서 해석할 여지가 있다. 여러 quantative and qualitative metric을 통해 T1 이미지로 생성한 FA 이미지가 T1 이미지보다는 실제 FA 이미지와 유사하다는 점을 보였다. 그러나 생성된 이미지가 PCA나 T-SNE의 결과 분포 상 실제 FA 이미지와 유사하더라도, image-to-image translation 과정에서 실제 T1 이미지에 생물학적 정보가 손상될 위험이 존재한다~\cite{Cohen2018-bi}. 만약 분포상 생성된 FA 이미지가 실제 FA 이미지가 육안상 유사하더라도, 중요한 개인차 정보가 손실된다면 임상적 가치가 심각하게 제한될 것이다. 생성된 FA 이미지가 실제 FA 이미지와 유사한 sex classification 성능을 보이는 것은 가장 기본적인 개인차인 생물학적 정보가 변환 과정에서 제대로 보존되었음을 의미한다. Macro2Micro는 실제 FA보다 성별 예측에서 더 높은 성능을 보이는데, 이는 T1을 FA로 변환하는 과정에서 생물학적 정보를 보존, 혹은 강화하는 방향으로 기능했음을 추론할 수 있다. 추가적으로 모델이 여러 subject를 학습하는 과정에서 scanner effect를 제거하는 효과가 존재해서 실제 FA 이미지보다 더 생물학적 특성이 두드러진 것으로 생각할 수 있다. 생성된 이미지에 대한 이러한 방식의 평가는 기존 생성 연구에서 자주 이루어지지 않았던 것으로, 실제 생성된 이미지를 활용하는 것이 높은 가치를 가짐을 시사한다. 차후에 성별 외의 다른 변수에 대해서 연구를 추가한다면, 생성된 이미지를 활용하고자 하는 연구자들에게 여러 유용한 가치를 제공해줄 수 있을 것이다.

% Compared to the predicted performance of the actual FA images, the higher or comparable sex classification performance of FA images generated by our Macro2Micro indicates the potential practical utility of the data in the future. However, even if the generated images show distributional resemblance to actual FA images in techniques such as PCA or T-SNE, there exists a risk of compromising biological information from the actual T1 images during the image-to-image translation process \cite{Cohen2018-bi}. 



Through various quantitative and qualitative metrics, it is demonstrated that the FA images generated from T1 images via the proposed model show high similarity with actual FA images, exceeding the similarity with T1 images. However, even if the generated images show a distributional resemblance to actual FA images in techniques such as PCA or T-SNE, there exists a risk of compromising biological information from the actual T1 images during the image-to-image translation process \cite{cohen2018distribution}. If the generated FA images result in the loss of important individual differences, the clinical application would be significantly limited. We demonstrated classification and regression performance in the generated FA images, which is similar to that of actual FA images. These similarities indicate that the fundamental individual biological information was conserved or amplified during the image translation process. Macro2Micro exhibits higher performance in predicting sex, intelligence and ADHD compared to actual FA, suggesting that it operated in a manner that preserved or enhanced biological information during the transformation from T1 to FA. Given that real T1, images exhibit superior predictive performance for sex, intelligence and ADHD compared to real FA images, we propose that the structural information present in T1 images was preserved and positively influenced the generated FA images. Furthermore, the heightened phenotype prediction performance of generated FA images might be attributed to their resilience against scanner effects. Training the model on multiple subjects can enhance its capacity to establish a consistent mapping between macro-structure and micro-structure. This robustness to versatile factors contributes to the emergence of more prominent biological characteristics in the generated images. Evaluation of generated images using such approaches has not been frequently conducted in previous generative research, emphasizing the high value of utilizing the actual generated images. If future studies extend their research to variables beyond sex, the utilization of generated images can provide researchers with various valuable benefits.
\\

% 한계점
% 우리 Macro2Micro는 학습하는 동안 모든 subject에서 동일하게 정 가운데 위치의 한 slice만 사용했기 때문에 brain의 끝 slice에 대해서는 좋은 성능을 보이지 못한다. 추후에 brain의 모든 slice를 넣고 학습시킨다면 좋은 퀄리티의 2d slice를 만들고 concatenate하여 realistic한 3d image까지 만들 수 있을 것이다.
% FA image로부터 Tractography를 예측하는 task에서의 결과는 다른 baseline model에 비해서 뛰어나지만 실제 tractography image와 비교했을 때 차이가 존재한다. 이 연구에서 macro structure로부터 tractography를 예측할 수 있음을 입증하였으며 deep learning을 통해 tractography를 image-to-image translation으로 만들어내는 연구의 장을 열었기에 앞으로의 연구에서 더욱 효율적으로 정확하고 정교한 이미지를 만들어나갈 수 있을 것이다.
% 상윰버전) 한편, Macro2Micro는 모든 subject에서 동일하게 z축을 기준으로 정 가운데 위치한 single slice만 사용하여 학습했기 때문에 z축의 끝부분에 있는 slice에 대해서는 좋은 성능을 보이지 못하였다. 추후 연구에서 brain의 모든 slice를 넣고 학습시킨다면 좋은 퀄리티의 2d slice를 만들고 concatenate하여 realistic한 3d image까지 만들 수 있을 것이다. FA image로부터 Tractography를 예측하는 task에서의 결과는 다른 baseline model에 비해서 뛰어나지만, 실제 tractography image와 비교했을 때 꽤 큰 차이를 보인다. 하지만, 우리는 본 연구에서 macro structure로부터 image-to-image translation으로 tractography를 생성할 수 있음을 입증하였기에 추가적인 연구를 통해 더욱 효율적으로 정확하고 정교한 이미지를 만들어나갈 수 있을 것으로 기대한다.

\textbf{Limitations.} On the other hand, in the Macro2Micro, only a single slice positioned in the middle along the z-axis was used for training. Consequently, it did not perform well on slices located at the ends of the z-axis. In future research, incorporating all slices of the brain and training the model could lead to generating high-quality 2D slices and concatenating them to create realistic 3D images. Although the results of predicting tractography from FA images outperformed other baseline models, there were still noticeable differences compared to actual tractography images. However, this study demonstrated the ability to generate micro-scale tractography from macro-structures using image-to-image translation. We anticipate that further research will enable us to create more accurate and sophisticated images efficiently.
\\

% 기대효과
\textbf{Future Impacts.} \textcolor{violet}{Stella : This research successfully generated microscopic structures from macro-structures of the human brain, demonstrating the interrelation between brain structures at different scales. Furthermore, it effectively learned subject-independent structures by accommodating individual variations.  In real-world medical settings, Macro2Micro has the potential to significantly reduce the time and cost required to obtain Diffusion Tensor Imaging (DTI). It can be effectively used for infants and patients with anxiety disorders who are unable to undergo time-consuming MRI procedures like DTI.}

This research successfully generated microscopic structures from macro-structures of the human brain, demonstrating the interrelation between brain structures at different scales. Furthermore, it effectively learned subject-independent structures by accommodating individual variations. In addition, when there is not enough time to scan various modalities in clinical practice, this approach enables translating different microscopic modalities from structural MRI, which is more readily obtainable. This significantly reduces the time required for diagnosis and decreases financial costs. Additionally, this approach facilitates multi-modality research by generating data for individuals who only have access to structural MRI or for populations where acquiring imaging data is challenging, such as pediatric patients.

% 이 연구는 macro structure로부터 microscophic structure를 생성해냈다. 이를 통해 scale에 따른 brain structure 사이에 연관성이 있음을 증명하였을 뿐만 아니라, 개인차 변이에 유연하게 학습하여 subject independent structure를 효과적으로 학습하였다. 또한, 임상에서 여러 modality를 촬영할 시간이 부족할 때, 얻기 어려운 microscophic structure를 structural MRI만 가지고도 알 수 있게 된다. 이를 통해 진단을 위한 시간이 상당히 축소될 수 있으며 금전적 비용도 감소할 수 있다. 또한, structural MRI modality data만 가지고 있는 환자 혹은 촬영하기 어려운 아동과 같은 사람들을 대상으로 data를 생성하여 multimodality 연구를 가능하게 한다.

% diffusion MRI같은 경우, 급성 뇌경색 진단에 가장 민감한 기법으로 발생 수 분 이내 병변이 나타나 초급성뇌경색의 치료 결정에 도움을 줄 수 있다. 그러나, 시간이 급박한 임상에서 두 모달리티의 이미지를 모두 촬영하는 데에는 많은 시간이 걸린다. 이를 smri 하나만 찍고도 dti를 만들어 함께 사용한다면 진단을 위한 시간이 상당히 축소될 것이다.
% smri 있던 기존 환자들의 데이터를 생성하여 multi-modal로 진단이나 연구에 필요한 데이터를 만들 수 있다.

% dwi만 가지고 fa를 만드는게 아니라 macro 정보인 smri를 함께 사용하면 더 잘되지 않을까?

==> redun./Supplementary__draft_.tex <==
The total intelligence score in the NIH toolbox was used for the intelligence prediction task. The parent KSAD (Kiddie Schedule for Affective Disorders and Schizophrenia) was employed as the diagnostic tool for assessing ADHD in children. Children who did not receive a diagnosis of KSAD and obtained a total problem score below 65 on the Child Behavior Checklist (CBCL) were designated as the healthy control group. We assessed the accuracy of classification tasks using FA images generated by CycleGAN, Pix2Pix, and Macro2Micro.

Additionally, we compared the predictive performance of these generated FA images with ground truth FA images or T1 images. Logistic regression with L2 norm was employed for gender classification, and PCA was used as the feature extraction method. PCA was applied to flattened, background-removed brain features, and feature reduction was performed by selecting the top 1,000 components (sex) and 500 components (Total intelligence, ADHD) that accounted for more than 90\% of the explained variance. The analysis was conducted on the test dataset of the image generation task. Among these datasets, 20\% were held out as a test set, while the remaining 80\% of the subjects were used for a training set in a 5-fold cross-validation. The models trained on these five folds were used to evaluate the performance on the held-out test set, and the results were averaged. Accuracy and AUROC were utilized for evaluating performances in classification tasks. Pearson product-moment correlation coefficients and mean square error (MSE) were chosen for evaluating the regression task.

\input{Table/norm_relu}

\textbf{Normalization \& Activation Function.}
Normalization and activation functions affect the quality of the generated images. In Table~\ref{tab:norm_relu}, we found that the normalization including batch normalization or instance normalization, and the ReLU activation function don't aid our Macro2Micro in synthesizing high-quality images. The combination of not using normalization and using leaky ReLU as an activation function performs the highest SSIM and PSNR scores and the lowest MAE and MSE scores. Also, the results using normalization or ReLU function have artifacts like dotted lines at the borders of the brain (Figure~\ref{fig:norm_relu}).

==> redun./intro_trash.tex <==
% A fundamental tenet of neuroscience states that the function of any component of the brain (including tissues, structures, and neuronal populations) is primarily determined by its connections \cite{friston2004functional}.
The human brain function is primarily determined by its connections. The brain consists of highly localized functioning of several brain regions and integration of these regions through neural connection~\cite{friston2004functional}.
%The brain appears to follow two basic principles of functional organization: 1) the assignment of certain brain regions to specific cognitive functions, and 2) the integration of these regions through neural connection \cite{friston2004functional}. Research studying the relationship between the brain's connectivity and the activation of specific brain regions during cognitive tasks has yielded novel understandings of the interplay between these two factors and how it affects human behavior.  In summary, the brain can be considered an ensemble of functionally specialized areas coupled nonlinearly by effective connections. 
The brain connections are constantly adjusted at systemic and synaptic levels to adapt to the ever-changing environment effectively. 
% The neuronal populations in the human brain adapt and transform themselves to cope with a constantly changing environment effectively.
Research studying the relationship between the brain's connectivity and its interplay with the environment has yielded novel understandings of adaptive human behavior. One important factor that makes the dynamic interaction possible is \textit{structural plasticity} at the macro and micro scale of the human brain.
%Influenced by innate genetic and epigenetic factors, brain connectivity is dynamically modified by activity or experience \cite{friston2004functional}. For example, during gestation, epigenetic mechanisms are prevalent. After birth, a higher focus is placed on activity- and experience-dependent plasticity. These alterations persist until adulthood, serving as a foundation for lifelong behavioral adaptability and learning via reorganization and plasticity reliant on experience.
 

The macro-structure of the human brain refers to the architecture of cell bodies and neurite arrangement within the gray matter or axonal properties (e.g., tissue organization, size distribution, density, and myelin content) in the white matter. The macro-structure of the human brain has enormous potential in understanding the structure and organization of the brain, providing unique insights for abnormalities that underpin disease states. The microstructure, on the other hand, refers to the microscopic structure of brain tissue components such as myelin, axons, and dendrites or the quantification of their properties. This microscopic structural architecture includes multiple properties such as cell size, the orientation of axonal fiber bundles, and packing density. Several dysfunctions of the human brain result from pathological features such as demyelination, inflammation, and axonal loss~\cite{cercignani2018brain}. As both macro- and micro-structure of the brain convey different yet complementary information of the human brain, considering both structures is extremely important for understanding the \textit{structural plasticity} of the human brain and connectivity during cognitive tasks.
\\

Magnetic resonance imaging (MRI) has had an unprecedented contribution to our understanding of the macro- and micro-structure of the human brain. 
%With the growing understanding of MR signals and hardware development, many MRI modalities reflecting different characteristics of the underlying anatomy have been proposed. 
The macrostructure of the brain could be captured by structural MRIs (sMRI), especially with T1-weighted MRI. T1-weighted images are favorable for observing macro-scale structures such as the overall shape and size of brain tissues. 
% Recently, research on Parkinson’s disease using sMRI found a correlation between memory dysfunctions and temporal lobe atrophy \cite{huisman2003diffusion}. Moreover, sMRI can be used for diagnosing psychiatric diseases such as ADHD and ASD. 
% brain development trajectory research and is the most used clinical imaging technology.
On the contrary, diffusion MRI (dMRI) can be used for studying brain tissue micro-structures \cite{gu2019generating}. Brownian motion of water molecules in the brain is restricted by factors such as the micro-environment and temperature \cite{ibarretxe2011brain} and this makes the properties of microscopic structural tissue can be observed sensitively at the voxel scale \cite{parker2004analysis}. Thus, dMRI is helpful in recognizing tissue damage or abnormalities that depend on the cell density of the tissue. Unlike sMRI, the contrast of the image in dMRI is determined by the difference in the diffusion rate of water molecules, so neuroanatomy can be seen at the function and physiology level \cite{ibarretxe2011brain}. Difussion-weighted Image (DWI), one of the most used in dMRI models can sensitively detect the increase in parenchymal signal due to tissue damage caused by cytotoxic edema for diagnosing hyperacute stroke. DWI is used in many advanced dMRI models such as neurite orientation dispersion and density imaging (NODDI), diffusion kurtosis imaging (DKI), and diffusion tensor imaging (DTI). In addition, diffusion-derived scalar maps provide rich information about micro-structural characterization \cite{gu2019generating}.

While these modalities have made great strides in identifying changes at different scale structures, they have generally proven to be very sensitive to tissue abnormalities, albeit with low specificity \cite{cercignani2018brain}. The multiplicity of factors contributing to the overall signal prevents a direct correlation between MRI biomarkers and biological substrate.

%Despite the impact that factors like myelin content and axonal packing have on the contrast, the multiplicity of factors contributing to the overall signal prevents a direct correlation between MRI biomarkers and biological substrate. 

To address the low specificity and embrace brain structures at different scales, several studies have attempted to combine multiple MRI modalities.  
% concerning multimodal MRIs have been proposed. 
% A multimodal study using T1 structural image and diffusion-weighted image (DWI) found an association between polygenic risk scores and hippocampal volume in Alzheimer’s disease \cite{ibarretxe2011brain}. Using T1, T2 (spin-spin relaxation), and DWI combined improves gender classification accuracy compared to when just one modality was used, leading to novel morphometric findings \cite{feis2013decoding}.
% Rethinking the macro- and microstructure of the human brain and the MRI techniques for capturing them, 
Diffusion tensor imaging (DTI) and T1-weighted images provide different yet complementary information. For example, DTI is particularly sensitive in reflecting the structural state of white matter, which has led to active research in white matter diseases such as multiple sclerosis \cite{horsfield1996apparent, roosendaal2009regional}, CADASIL \cite{chabriat1999clinical, o2005damage}, amyotrophic lateral sclerosis \cite{segawa1994mri, muller2016large}, and Alzheimer's disease \cite{mayo2019relationship, chen2023abnormal}. These studies have demonstrated that DTI can effectively detect pathological alterations in white matter regions that appear normal in T1 and that changes in DTI measures correlate with pathological changes and clinical findings.


%T1 captures information about various tissues related to the brain's macro-structure, such as grey matter, white matter and cerebrospinal fluid. DTI, on the other hand, captures information regarding the micro-structure of white fiber tracts' distribution. DTI is particularly sensitive in reflecting the structural state of white matter, which has led to active research in white matter diseases such as multiple sclerosis \cite{horsfield1996apparent, roosendaal2009regional}, CADASIL \cite{chabriat1999clinical, o2005damage}, amyotrophic lateral sclerosis \cite{segawa1994mri, muller2016large}, and Alzheimer's disease \cite{mayo2019relationship, chen2023abnormal}. These studies have demonstrated that DTI can effectively detect pathological alterations in white matter regions that appear normal in T1 and that changes in DTI measures correlate with pathological changes and clinical findings.

Therefore, a multimodal approach that simultaneously utilizes DTI and T1 allows for a more comprehensive understanding of brain information, as recent research supports. Recently, the fusion of diffusion indices and surface information through T1-DTI fused images has shown improved detection power in distinguishing between individuals with mild cognitive impairment (MCI) and healthy controls \cite{lao2017t1}. Furthermore, a multimodal approach incorporating feature selection from both T1 and DTI data has demonstrated superior performance in age regression compared to the unimodal approach, which utilizes each data modality separately. \cite{cai2023brain}.

Similarly, research to use tractography, which can capture brain connection information, is also in the spotlight. Fractional anisotropy (FA) is the most widely used quantitative index obtained through DTI. However, the FA image has a single scalar value for each voxel. Thus it cannot represent the directionality of tissues in each voxel. On the other hand, tractography utilizes DTI data to tract and reconstruct fiber pathways, providing insights into the structural connections between different brain regions. By tracing the trajectory of neural fibers, tractography can effectively capture and visualize the connectivity patterns in the human brain, which FA alone cannot achieve. Considering and analyzing these three MRI modalities all at once would be a milestone in neuroscience in that each of them provides distinct yet complementary information. \\

%Moreover, several studies showed that tractography is highly correlated to human phenotypes. Differences were found in 25 distinct fiber bundles between ADHD patients and the healthy control group \cite{hong2014connectomic}. 

%In addition, abnormalities in tractography of the frontal cortex were found in bipolar disorder \cite{lin2011abnormal}. Tractography has also been used to construct the topological organization of the human cortical anatomical network and investigate differences between sexes \cite{yan2011sex}. Due to its strong correlation with factors such as human sex and diseases, tractography can be applied in clinical fields for diagnosis and other purposes. 

%%%%%%%%%%%%%%%%%%%%%%%%%%
%% multi-modal 왜 잘 안되었었는지 --> 일단 쒸바 구하는게 졸라 어렵다. dwi 같은 경우 어떻게 어렵고 dti는 어떻게 어렵고, tractography는 어떻게 어렵다. 개개별로 구하는 것도 어려운데 이 세개를 동시에 얻는거는 사실상 잘 없다. 그래서 이런 점이 multimodal 연구를 막던 가장 큰 장애물이었다.
% 준우야 single modality 구하는 게 어려운 건 여기보다 다른 데 더 어울리는 내용 같아서 여기서는 multimodality가 어려운 이유에 대해서 쓸게!! -상윤
% 각 modality가 뇌의 각기 다른 조직을 다른 scale에서 나타내기 때문에 modality마다 표상하는 정보가 다르다. 그래서 이를 통합하기 위한 multimodal 연구가 많이 시도되었는데, neuroimage에 있어서 multimodal deep learning은 여러 가지 challenge를 수반한다. 많은 양의 데이터가 중요한 딥러닝 과제에서 모든 modality를 가지고 있지 않은 subject는 분석에서 제외해야 하기 때문에 데이터의 개수가 줄어들 수 밖에 없다. 이는 곧 generalizability의 감소, overfitting 위험의 증가를 낳는다. 또한, multi modality data를 효과적으로 통합하기 위해서는 이들의 상호작용을 잘 표현해야 하는데, 이 때 복잡한 model architecture를 필요로 하며, 결과적으로 더 많은 계산 리소스와 학습 데이터를 필요로 한다. 

%Because each modality represents different aspects of brain tissue at different scales, the information captured by each modality is inherently different. 

There have been numerous attempts to integrate these modalities in a multimodal fashion in neuroimaging studies. However, multimodal deep learning poses several challenges.

% 1 치료적으로 장시간 촬영이 어려운 이들에게(clinical practice) - 이것을 15분 이상 찍는 게 현실적으로 어려운 사람들에게 많은 도움을 줄 수 있다 (3? 4? 문단)
% 아래 문단의 국문 초안 버전입니다 -상윤- DTI는 T1에 비해 촬영 시간이 훨씬 길다. 우리가 이용할 ABCD (Adolescent Brain Cognitive Development) 데이터에서도 DTI의 기반이 되는 DWI (Diffusion weighted imaging)는 이미지를 얻는 데 7분 30초 걸렸고 (상윤 혹시 이거 dwi 1개 찍을때 하는거지? 응! 아아 오키 dti 찍을때 최소 6개 이상 dwi 쓰거든? 그래서 dti(fa) 구하는거 시간을 적어주면 더 극적일거같아->그거까지 계산해서 넣을게 요거 확실하게 논문에서 찾아서 넣어주라!! 왜냐면 프로토콜 마다 6개 쓰는 애들도 있고 뭐 더 많이 쓰는 애들도 있음 최소 6개야 (내가 알기론))->ㅇㅋㄷㅋ, T1은 Phillips scanner를 기준으로 촬영을 하는 데 5분 38초 걸렸다\cite{casey2018adolescent}. 환자가 긴 시간 동안 MRI scanner 안에 긴 시간을 있어야 T1과 DTI를 동시에 얻을 수 있다. 하지만, MRI scanner의 환경 자체가 스트레스를 불러일으킬 수 있기 때문에 panic disorder나 agoraphobia가 있는 환자군에서 (PD/AG) MRI의 품질이 저하된다는 연구가 발표된 바 있다\cite{lueken2011don}. 또한, MRI scan은 움직임에 매우 민감하여 움직임이 잦은 영유아의 경우에는 진정제나 마취제를 투여하기도 하지만, 윤리적인 이유와 잠재적인 장기 위험 때문에 상기 방법은 권장되지 않는다\cite{copeland2021infant}. 따라서 오랜 시간 MRI scanner 안에 머무를 수 없는 환자들이나 움직임이 잦은 유아들은 DWI처럼 오랜 시간이 걸리는 영상을 고품질로 얻기는 현실적으로 불가능하다.
The major bottleneck for multimodal studies is that obtaining different modalities data is \textit{extremely} costly and time-consuming. For example, Diffusion Tensor Imaging (DTI) requires a much longer acquisition time compared to T1-weighted imaging. In the ABCD (Adolescent Brain Cognitive Development) dataset we utilized, obtaining the DWI (Diffusion Weighted Imaging) data, which serves as the foundation for DTI, took 7 minutes and 30 seconds per single subject. Also in the ABCD study, to obtain a single DTI (Diffusion Tensor Imaging) image, 96 DWI (Diffusion Weighted Imaging) images are required \cite{hagler2019image}. Therefore, it would take approximately 720 minutes to acquire DTI images for a single patient, while T1 imaging took 5 minutes and 38 seconds using a Phillips scanner \cite{casey2018adolescent}. To obtain both T1 and DTI images simultaneously, patients need to remain inside the MRI scanner for an extended period. However, studies have shown that the quality of MRI scans can be compromised in patients with panic disorder or agoraphobia (PD/AG) due to the potentially stressful nature of the MRI environment \cite{lueken2011don}. Additionally, MRI scans are highly sensitive to motion, leading to the use of sedatives or anesthesia in infants with frequent movement. However, these approaches are not recommended due to ethical concerns and potential long-term risks \cite{copeland2021infant}. Therefore, it is practically impossible to obtain high-quality images for lengthy acquisitions like DWI in patients who cannot tolerate long periods inside the MRI scanner or in infants with frequent motion.

Moreover, when it comes to obtaining tractography, generating 1 million tracks using software such as MRtrix3\cite{tournier2019mrtrix3} typically takes around 12 hours per subject. Such challenges significantly limit the clinical applicability of tractography despite its potential value. Recently, research generating tractography from diffusion-weighted imaging (DWI) has started to emerge, and even that remains rare \cite{benou2019deeptract}.


% 1 만들어낸 이미지가 좀 더 noise에 robust하고, general한 특성을 잘 학습할 수 있다

% 2 딥러닝 모델 학습에서도 딥러닝은 항상 데이터의 수를 많이 필요로 하는데, 이러한 학습 데이터의 증강을 통해 학습을 촉진할 수 있다.
In deep learning research where a large amount of data is crucial, only subjects who have data for all modalities can be used for the analysis. As a result, the available data size is inevitably reduced. It can lead to decreased generalizability and an increased risk of overfitting. Furthermore, effective integration of multimodal data requires capturing their interactions accurately, which often necessitates complex model architectures and, consequently, requires more computational resources. This study seeks to propose a model that can generate FA and tractography from T1 without requiring a significant amount of time and resources.
\\
%Many studies that utilize multimodal data operate under the assumption that the imaging signals have the same neuronal origin. However, it is worth noting that differences can exist in the parameters used to acquire the images and how neuronal processes and structures contribute to the imaging signals \cite{uludaug2014general}.


% 요새는 이 문제를 i2i translation으로 풀더라! (이후로 i2i 설명)
%%%%%%%%%%%%%%%%%%%%%%%%%%
%DWI is used in many advanced dMRI models like neurite orientation dispersion and density imaging (NODDI) and diffusion kurtosis imaging (DKI) or diffusion tensor imaging (DTI). Recently, advanced dMRI models need high-quality and various image signal intensity options of DWI [7]. As tissues with active/inhibited diffusion motion depend on the b-value, various b-values are needed to detect as many lesions as possible. However, raw DWI quality is relatively poor due to low signal-to-noise ratio, long echo times, and long repetition times [5]. A prior study translated sMRI and b0 image to DWI in high-quality and dense q-space diffusion MR images using deep learning [7]. They mainly focused on generating lost or damaged DWI images using obtained DWI. The research proved that data-driven deep learning generates realistic DWI.

%%%%
%Diffusion MRI is a non-invasive technique used for studying brain tissue microstructures. Diffusion-derived scalar maps provide rich information about microstructurl characterization, but there are two major bottlenecks in obtaining these sclar maps. First, it is expensive and time consuming to acquire high quality diffusion data. Since MRI scanners are sensitive to motion, it is challenging to obtain high-quality MRI data from children due to their tendency to move inside the scanner. Therefore, it is realistically challenging to acquire high-quality MRI data from children \cite{copeland2021infant}. Second, the accuracy of the diffusion-derived scalar maps relies on elaborate diffusion data processing pipelines, including preprocessing (head motion, eddy current distortion and susceptibility-induced distortion corrections), diffusion model fitting and diffusion scalar calculation. Small errors occruring at any of these steps can contribute to the bias of the diffusion-derived scalars. For adolescent, such steps can take hours to finish.




% 그런데! micro 자체가 macro로부터 예측할 수 있음이 최근들어 주목받고 있다. 이러한 태스크는 주로 T1으로부터 FA나 MD이미지를 예측하는 방식으로 이루어 졌다. 이러한 연구들에서는 주로 GAN이나 translation 모델 등을 활용해서 이러한 비선형적인 둘의 관계가 학습될 수 있음을 밝혀왔다.
% 근데 그 개개인의 뇌 구조를 가르는 개인차 정보는 모두 macro안에 존재하기에, 이것으부터 micro structure까지도 예측할 수 있음이 기존 연구들을 통해 검증되어왔다. (T1 to FA 연구들을 인용)  - rationale 필요.
%- macro 정보(T1)에 micro 정보가 담겨있다는 내용
% 모델 구조를 뒷받침하는 rationale. (style이라는 것이 결국 개인차다.)
% 개인차가 존재하는데, 이것을 정확하게 개개인의 micro 구조로 translation할 수 있다는 것이 밝혀져 있다. (ref 필요)



%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%

%%% 이부분은 i2i 들어갈때 써먹으면 좋을 문장
%One way to address this question exploits deep learning algorithms, which have revolutionized the analysis of neuroimaging data in the past two decades.


% To address, Image-to-image translation 접근의 효과성 그리고 한계 - 1문단
% ItoI 에 대한 간단한 배경 및 그것의 가치 - 어떤 태스크에서 유용하게 쓰일 수 있고, 뇌 연구에서 이것들이 어떤 발견들을 이루어냈는지? - harmonization 연구들, T1 to DTI, GANDALF - 임상적으로 치매 예측한 연구, GANBERT, Image reconstruction해서 손상된 데이터를 복원하는 연구.  % T1 to FA 연구를 직접적으로 설명하면서 그것들의 한계를 서술. (CycleGAN-무작정 translation을 하면 성별 등 데이터 분포를 의도치 않게 바꿔버릴 수 있다.) - Cycle-consistent loss, 임상적인 가치를 다룬 연구가 거의 없다. - 생물학적 특성이 translation 전후에 얼마나 변화하였는지를 분류 태스크를 통해 검증하고자 한다. 

% Tractography는 FA와는 구별되는 더 micro한 정보를 담고 있으며, 이것을 얻는 것은 매우 어렵다.% 연구적으로 활용할 순 있지만 임상적으로 Tractography를 활용하는 경우가 매우 드물다. 
% Tractography를 실제로 뽑는 데에는 ~~정도의 시간이 걸리며 (얼마나 걸리는지에 대한 rationale) ; 서영이 피셜 인당 12시간이래
% 실제로 그러한 이유로 기존의 방법론 ~~~ 이후로 딥러닝을 이용해 이것을 개발하는 접근은 매우 드물었다.
% 그래서 본 연구는 이러한 접근을 end-to-end manner로 직접적으로 예측하고자 한다. 일반적으론 이런데 현실적으론 이렇게 바꿨다 ...이런 접근을 취하려고 한다)
% 상윰초안 - 하지만 mrtrix 등의 소프트웨어를 이용해 tractography를 생성하는 데는 1 million track을 기준으로 한 명의 subject 당 12시간이 걸리기 때문에 임상적으로는 충분한 가치가 있음에도 불구하고 현실적으로 많이 사용하지 않았다. 최근이 되어서야 DWI로부터 tractography를 만드는 연구가 시작되었고, 이마저도 매우 드물었다 \cite{benou2019deeptract}. 그래서 본 연구는 오랜 시간을 들이지 않고도 tractography를 생성할 수 있는 모델을 제안하려 한다.

% 잘되면? - 1문단 (임상적 가치/효과)




% 또한 최근에 뇌의 frequency에 따라 구조에 있어서 구분되는 정보를 얻을 수 있음이 밝혀졌다. % low frequency는 high level 정보를, high frequency는 뇌 영상의 low level 정보를 담고 있다.  각 정보는 임상적으로 어떠어떠한 질병을 예측하거나 구분하는 특성을 가짐이 밝혀졌다. (-배상윤 - 얘들아 근데 내 논문은 fMRI 관련이거든. 기본적으로 timeseries 데이터를 frequency domain으로 옮긴 다음에 low frequency는 이런 시스템이고 high frequency는 저런 시스템이고 이런 논리 전개가 되는데 여기에 적용할 수 있을까,,,수영준우준범 셋 다 내 논문 접근 권한 있지?) 그리고 또한 frequency를 구분하는 것이 생성 태스크에서도 효과적으로 정보를 뽑아낼 수 있음이 밝혀졌다. - AesFA 참고. 뇌영상에서도 이러한 접근이 충분히 효과적이라고 추론할 수 있다. (이미 이런 접근이 있다면 무조건 인용.)

%% 아래는 내가 divfreqBERT 에서 썼던 부분.. 아무래도 T1 DTI 논문에는 맞지 않는 듯 함.
%Recently, methods have been developed to analyze fMRI timeseries by dividing them into frequencies using clustering. Sasai et al.\cite{sasai2021frequency} discovered that regions with similar frequency spectra, as detected using fast fMRI, correspond to the regions forming functional modules in the brain network. They also found that different frequency bands contribute to neural interactions in distinct ways during task execution. Kajimura et al.\cite{kajimura2023frequency} demonstrated that the BOLD (blood-oxygen-level-dependent) signals of resting-state fMRI exhibit frequency-specific network structures, revealing that the network architecture changes with frequency. These methods suggest that using frequency as a basis to separate fMRI data into functional modules or distinct brain dynamics is reasonable in order to enhance our understanding of the data.

%% Stella wrote about the frequency dividing approach in the brain... 아래 내용도 다 포함해서 썼어
A recent study has shown that when structural brain imaging is divided into high-frequency and low-frequency components, the performance in the image reconstruction task is better compared to the cases without frequency division \cite{nguyen2019frequency}. Similarly, encoding and decoding the brain based on its frequencies could significantly increase the quality of synthesizing the target image. This study aims to develop a novel image-to-image translation model, Macro2Micro, that can be applied to the brain, utilizing octave convolution commonly used in computer vision.

Firstly, we compare and validate our proposed model rigorously against existing studies in the T1 to FA image translation task. Furthermore, we extend our research by generating tractography from the FA images, allowing us to explore the potential of our model in capturing and representing the structural connectivity information of the brain.\\

% 나열식으로 쓰지 말고 논설문으로 쓰는 것 - 하고 싶은 말은 frequency를 다룬 연구들을 통해 뇌를 frequency에 따라 encoding하는 우리의 접근이 설득력이 있다 라는 것을 어필하는 식으로 써야함.
% Octave convolution은 하나의 예시로서 다룰 것 (Computer vision 사례에서)

% 본 연구에서는 이러한 차원에서 기존의 Computer vision 도메인에서 쓰이는 방법들을 기반으로 새로운 Image Generation 모델을 개발하고자 한다. 먼저, T1 to FA translation task에서 기존 연구들과 비교하며 좀 더 면밀하게 검증하고자 한다. 더 나아가, 생성된 FA로부터 tractography를 생성하는 태스크까지 해보려고 한다.

% 기존에는 이것에 대해서 면밀하게 (metric 적으로, clinically) 검증이 이루어지지 않았고, 개인차의 존재성에 대해 별로 주목하지 않았다.  %mode collapse 등 개인차를 소실하는 GAN의 이슈에도 불구하고 이러한 점을 고려하지 않았다.

% 이걸 통해 결과 highly synthesized image with increasing performance by OO% compared to the other algorithm.

%%%%% 

% Ablation으로 보고 싶던 것들을 Discussion에서 서술
% VGG 쓰면 좋다 라는 건 result --> Discussion에서 VGG의 plausible한 역할을 서술 (뇌과학적으로)
% Octave도 Discussion에서 왜 이 태스크에 도움이 되는지를 나름대로 해석




%Diffusion에서 예측할 수 있는 정보들 --> 생물학적 정보들

% Frequency에 대한 정보들

% Image-to-image translation for T1(macro) to FA (micro)





\section{Related work} 

\textbf{Modalities in Neuroimaging.} Magnetic Resonance Imaging (MRI) is a non-invasive imaging technology that produces three-dimensional detailed anatomical images. It is often used for disease detection, diagnosis, and treatment monitoring. It is based on sophisticated technology that excites and detects the change in the direction of the rotational axis of protons found in the water that makes up living tissues. Structural MRI, in particular, provides high-resolution, three-dimensional images of the brain's anatomy. It is commonly used to visualize the brain's structure and detect abnormalities such as tumors, strokes, or developmental anomalies. T1-weighted imaging (T1) is a specific type of MRI that uses the longitudinal relaxation time of tissues to produce images. T1 is particularly useful for visualizing anatomy and pathology in high detail, making it a valuable tool in neuroimaging. \par

Diffusion Tensor Imaging (DTI) is a type of MRI that measures the random motion of water molecules within a voxel of tissue. It is particularly useful for visualizing white matter tracts in the brain, as the direction of water diffusion can provide information about these fibers. Fractional Anisotropy (FA) is a scalar value between zero and one that describes the degree of anisotropy of a diffusion process. A value of zero means that diffusion is isotropic, i.e., it is unrestricted (or equally restricted) in all directions. A value of one means that diffusion occurs only along one axis and is fully restricted along all other directions. FA is a commonly used measure in DTI studies, as it can provide important information about the integrity of white matter tracts. \par

In addition to FA, another commonly used measure in DTI is Mean Diffusivity (MD). MD represents the average magnitude of water diffusion within a voxel, regardless of direction. It is a scalar value that reflects the overall diffusion characteristics of the tissue. Higher MD values indicate greater diffusion, suggesting less restriction or damage to the tissue. Conversely, lower MD values indicate reduced diffusion, which may indicate more restricted or compacted tissue. MD is often used in conjunction with FA to provide a more comprehensive understanding of the microstructural properties of matter tracts. By combining information from both FA and MD, researchers can gain insights into the structural integrity and health of the brain's white matter pathways. \par

Tractography is a 3D modeling technique used to visually represent neural tracts using data collected by diffusion MRI. It uses special techniques to visualize, analyze, and quantify the diffusion of water molecules in the white matter of the brain, which can provide insights into the structure and connectivity of the brain's neural pathways. Tractography can be used to generate a detailed map of the brain's white matter tracts, which can be useful in neurosurgical planning, diagnosing various neurological conditions, and understanding the brain's connectivity. It can be performed in 2D slices or as 3D reconstructions, providing a comprehensive view of the brain's white matter architecture. \\

\textbf{Image-to-Image Translation.} Image-to-image translation refers to the task of converting an input image from one domain to another while preserving relevant visual information. It aims to learn a mapping function to transform images from a source domain to a target domain, enabling various applications such as style transfer, colorization, and modality conversion. Its goal is to generate realistic and visually coherent output images that are indistinguishable from the target domain. \par
Despite advancements in image-to-image translation, several challenges persist. These challenges include:
\begin{itemize}
    \item \textbf{Paired Data Requirement}: Many existing methods rely on paired training data, where corresponding images from the source and target domains are required. However, obtaining such paired data can be time-consuming and expensive in certain domains.
    \item \textbf{Mode Collapse}: Some algorithms may suffer from mode collapse, where the generator produces limited variations of the target domain, resulting in a lack of diversity in the generated images.
    \item \textbf{Preserving Fine Details}: Preserving fine-grained details during the translation process can be challenging, especially when the input and output domains have significant differences in texture, shape, or resolution.
\end{itemize} \par
To address the above challenges, several image-to-image translation algorithms have been proposed. Pix2Pix \cite{isola2017image} is a conditional generative adversarial network (cGAN) that learns a mapping from input images to output images using paired training data. It combines a generator network with a discriminator network to optimize the image translation process. It produces high-quality translations when trained with paired data and can preserve fine details. However, it heavily relies on paired training data, which can be a limitation in certain scenarios. 

CycleGAN \cite{zhu2017unpaired} is an unsupervised learning approach that utilizes cycle consistency to learn mappings between two domains without paired data. It introduces cycle consistency loss, which enforces the reconstructed image to be close to the original input, ensuring consistency in both directions. It does not require paired training data, making it more flexible for real-world applications. However, it may struggle with preserving fine details and can be sensitive to hyperparameter settings. \par

% \textbf{UNIT} (Unsupervised Image-to-Image Translation) is an unsupervised approach that aims to learn a shared latent space between two domains (Liu et al., 2017). It employs a shared-latent space assumption, allowing the model to translate images between domains without paired data. It can perform image-to-image translation without paired data, making it applicable to various domains. However, it may face challenges in capturing complex mappings between domains and can be computationally expensive. \par
These algorithms represent significant advancements in image-to-image translation, each with its own strengths and limitations. Further research and exploration are necessary to address the challenges and improve the performance of cross-modality image-to-image translation techniques. \\

\textbf{Structure MR Image to Diffusion Tensor Image Translation.} 
Gu et al. \cite{gu2019generating} explored the use of GANs, specifically CycleGAN, to generate synthetic diffusion scalar measures from structural T1-weighted images. This approach aimed to address the challenges of cost and time consumption in collecting high-quality diffusion data and the complexity of diffusion data processing pipelines. The CycleGAN model was trained to map a T1 image to FA or MD, and vice versa. The synthetic FA images were then used as a target for non-linear registration to correct for geometric distortions common in diffusion MRI. The results showed good to great visual similarity between synthetic FA and MD images and their ground truth, with the trained CycleGAN performing well across all test subjects. However, the authors noted that the training data used could influence the GAN's performance, potentially introducing bias. \par
Yang et al. \cite{Yang2020CMI2I} proposed a cross-modality generation framework that leverages cGANs for Image Modality Translation (IMT) in MR images. The framework was designed to exploit both low-level features (pixel-wise information) and high-level representations (e.g. brain tumors, brain structure) between cross-modalities, addressing the complexity of brain structures. The authors introduced an end-to-end IMT network for cross-modality MRI generation and provided a comprehensive comparison with five datasets representing real-world clinical applications. \par

The paper also presented two novel methods that utilize the IMT framework. The first was a registration method that augments the fixed image space with translated modalities for atlas-based registration. The second was a segmentation approach, called translated multichannel segmentation (TMS), which performs cross-modality image segmentation using fully convolutional networks (FCNs). Both methods leverage cross-modality information to improve performance without the need for additional data. \par

Despite achieving excellent performance, the authors acknowledged that the generated images may not accurately represent tiny structures as compared to real images. \par
Anctil-Robitaille et al. \cite{anctilrobitaille2020manifoldaware} proposed a novel approach to image-to-image translation for manifold-valued data, specifically in DTI, using a manifold-aware CycleGAN. Traditional GANs have been limited in their application to DTI due to their non-Euclidean nature. The authors addressed this by formulating the objective as a Wasserstein distance minimization problem of data distributions on a Riemannian manifold of symmetric positive definite 3x3 matrices (SPD(3)), using adversarial and cycle-consistency losses. They leveraged the Log-Euclidean metric and the structural information of T1-weighted (T1w) images to generate realistic high-resolution DTI. The generated diffusion tensors were ensured to lie on the SPD(3) manifold by exploiting the theoretical properties of the exponential and logarithm maps of the Log-Euclidean metric. \par

The proposed method outperformed both the manifold-aware GAN and the standard CycleGAN in terms of tensor principal orientation estimation, Log-Euclidean distance, and mean squared error (MSE) of derived FA. The results suggested that T1w images may contain information on the high-level geometry of fiber tracts, which can be learned by the network to estimate the diffusion properties and orientation. This work represents a significant contribution to medical image computing, unlocking a vast number of applications on manifold-valued data. \par

Liu et al. \cite{Liu2023Attentive} developed a generative self-training (GST) framework for unsupervised domain adaptive (UDA) medical image translation tasks. The framework incorporates a unified uncertainty quantification scheme for both epistemic and aleatoric uncertainties, allowing for adaptive control of generative pseudo-label supervision based on the reliability of the pseudo-labels. This approach was applied to tagged-to-cine and structure-to-diffusion (e.g., T1-to-FA) image translation tasks, marking the first attempt at such UDA. The results demonstrated superior translation performance compared to popular adversarial UDA methods. The framework also includes a self-attention scheme to emphasize regions of interest and prevent the background region from dominating the training process. The authors also noted that their framework could be applied to other discriminative self-training UDA tasks and that different backbones in the source and target domain could be used. \\

\textbf{Anatomy of the Brain and the vmPFC.}
The human brain is divided into several distinct regions with specific functions and responsibilities. Major divisions of the brain include the cerebrum, cerebellum, and brainstem. The cerebrum, the largest part, is further divided into two hemispheres and is responsible for higher brain functions such as thinking, learning, and consciousness. Each hemisphere is divided into four lobes: the frontal lobe (responsible for reasoning, problem-solving, and skills), the parietal lobe (processing sensory information), the occipital lobe (vision), and the temporal lobe (hearing and memory). Understanding the intricate structure and function of the brain is essential for developing effective image-to-image translation techniques in brain imaging. \par

The ventromedial prefrontal cortex (vmPFC) is a subregion of the prefrontal cortex, located in the anterior part of the brain. It is situated where the two cerebral hemispheres meet at the bottom (ventral) part of the frontal lobes, hence its name. The vmPFC is bounded by the orbital prefrontal cortex (OFC) laterally, the anterior cingulate cortex (ACC) dorsally, and the subgenual cingulate cortex (sgACC) posteriorly. \par

The vmPFC is a complex and heterogeneous region with diverse cytoarchitectonic features, indicating a variety of functions. The vmPFC has extensive connections with other brain regions, including the amygdala, hippocampus, hypothalamus, and various sensory areas, which facilitate its role in integrating emotional, cognitive, and sensory information. \par

The vmPFC is not only involved in decision-making and emotional processes but also plays a role in self-referential thinking and theory of mind–the ability to understand other's mental states. It is also implicated in the regulation of autonomic and endocrine responses to stress, and the formation and retrieval of personal memories. \par

In neuroimaging studies, the vmPFC is often challenging to image due to its location and susceptibility to signal dropout. However, accurate imaging of the vmPFC is crucial given its involvement in various cognitive processes and its implication in numerous psychiatric and neurological disorders. Therefore, advanced image-to-image translation techniques that can accurately capture the structure and function of the vmPFC are of great importance in neuroscience research. \\


\textbf{Frequency-based Brain Analysis.} Data obtained from brain function measurements, such as EEG (Electroencephalography) and fMRI (Functional Magnetic Resonance Imaging), can be divided into multiple frequency bands. EEG data is characterized by electrical activity in the brain, and it can be divided into different frequency bands to examine different aspects of brain function. The commonly recognized frequency bands in EEG analysis are delta, theta, alpha, beta, and gamma. Delta (0.5-4 Hz) frequency is the lowest frequency range, primarily observed during deep sleep. Theta (4-8 Hz) frequency is primarily observed during sleep but can also be associated with altered states of consciousness. Alpha (8-13 Hz) frequency is typically observed during relaxed states, such as when closing the eyes and resting. Beta (13-30 Hz) frequency is predominantly observed during wakefulness and is associated with alertness. Gamma (30-100 Hz) frequency is a higher frequency range associated with complex brain activities related to cognition, attention, and memory \cite{klimesch1999eeg, bacsar2001gamma, buzsaki2004neuronal}. These frequency bands help us understand the characteristics of EEG signals and investigate various aspects of brain activity. Frequent band changes can be used to track changes in brain function related to cognition, sleep, attention, and other processes.

On the other hand, fMRI measures changes in blood oxygenation levels to infer brain activity. Although fMRI does not directly provide frequency information like EEG, researchers can analyze fMRI data to study the functional connectivity and fluctuations in different frequency ranges. Resting-state functional MRI research has uncovered that the blood oxygen level-dependent (BOLD) signal in the brain shows slow intrinsic fluctuations (less than 0.1 Hz) that are correlated over time. These fluctuations indicate a relationship within hierarchically organized functional systems known as resting state networks \cite{doucet2011brain}.

Furthermore, when applying a fast Fourier transform to fMRI data and examining it in the frequency domain, the scale-free activity demonstrates a division into frequency bands based on the knee frequency of the Lorentzian function \cite{diba2004intrinsic, miller2009power}. The presence of a low-frequency band suggests that the system exhibits decreased temporal redundancy and operates more efficiently in processing information in real time. Conversely, the high-frequency band indicates a higher level of time-lagged auto-correlation, indicating that past dynamics of the system have a greater impact on its future dynamics, thereby indicating the presence of long-range memory effects \cite{eke2002fractal}.

Different frequency ranges in brain signals correspond to different functional systems within the brain. This means that different functions generate signals in different frequency ranges. Therefore, analyzing brain research data by dividing it into frequency bands can help to elucidate various brain functions more clearly.




%%%%

In summary, the main contributions of this research encompass:
\begin{itemize}
    \item We propose a novel I2I translation framework, Macro2Micro for synthesizing diffusion MRI and tractography from structural MRI. Our model achieves the highest quality compared to various I2I algorithms qualitatively and quantitatively.
    \item To effectively synthesize the brain MR images, we introduce several simple yet effective modifications on the discriminator, yielding more satisfying output with fine brain details. To further accelerate the networks' capability to learn subject-independent representation and the connectivity between the macro and micro-structure, Octave Convolutions and prior knowledge from pre-trained convolutional neural networks are used. Comprehensive experimental results demonstrate the validity of our design choice and its superiority to conventional I2I translation techniques.
    \item To the best of our knowledge, this is the first attempt to translate tractography from structural MR images in medical image modality translation scenarios.
\end{itemize}
